Planning for Goal-Oriented Dialogue Systems

Generating complex multi-turn goal-oriented dialogue agents is a difficult problem that has seen a considerable focus from many leaders in the tech industry, including IBM, Google, Amazon, and Microsoft. This is in large part due to the rapidly growing market demand for dialogue agents capable of goal-oriented behaviour. Due to the business process nature of these conversations, end-to-end machine learning systems are generally not a viable option, as the generated dialogue agents must be deployable and verifiable on behalf of the businesses authoring them. In this work, we propose a paradigm shift in the creation of goal-oriented complex dialogue systems that dramatically eliminates the need for a designer to manually specify a dialogue tree, which nearly all current systems have to resort to when the interaction pattern falls outside standard patterns such as slot filling. We propose a declarative representation of the dialogue agent to be processed by state-of-the-art planning technology. Our proposed approach covers all aspects of the process; from model solicitation to the execution of the generated plans/dialogue agents. Along the way, we introduce novel planning encodings for declarative dialogue synthesis, a variety of interfaces for working with the specification as a dialogue architect, and a robust executor for generalized contingent plans. We have created prototype implementations of all components, and in this paper, we further demonstrate the resulting system empirically.

==> cache/executor_cache.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/execution_monitor_cropped6.pdf}
    \caption{Architecture for executing contingent plans.}
    \label{fig:architecture}
\end{figure}

\section{Plan Executor}
\label{sec:exec}

Our aim here is to provide a coherent and effective strategy for deploying dialogue agents that are based on the execution of a contingent plan. In this section, we identify some of the key challenges that arise in building an executor of such plans and propose a solution to each of them.
The high-level architecture we propose is in Figure \ref{fig:architecture}. The execution involves the following phases:

\begin{enumerate}
    \item At every iteration of the execution monitor, we have the state of the world (relevant to the planner), a context of variable assignments (used by the executor, not needed by the planner), and the plan's current node $n$ along with the corresponding action $a = \actmap{n}$.
    \item The executor retrieves the relevant context and state for action $a$ (Section \ref{ssec:exec-vs-det}).
    \item The action execution function ($\exec{a}$) is called with the filtered context.
    \item The action's effect is determined (Section \ref{ssec:complex_outcome_determination}).
    \item The state and the context are updated (Section \ref{ssec:complex_outcome_determination}).
\end{enumerate}

% General Framework
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/execution_monitor_cropped5.pdf}
%     \caption{Architecture for executing contingent plans.}
%     \label{fig:architecture}
% \end{figure}


To motivate the type of complex actions we wish to execute, consider an example scenario where a virtual agent can perform common tasks around the household. Figure \ref{fig:pddl-example} shows an example PDDL representation of an action which prepares the garage for a car to exit, and Figure \ref{fig:effect-example} shows the accompanying effect structure. Notice that some of the non-determinism is independent (e.g., the locked status of the garage door and the alarm status), and some of the non-determinism contains a dependency (e.g., the open status only plays a role when the door is not locked). We address these points further in the following sections.



\begin{figure}[t]
\centering
\begin{BVerbatim}[commandchars=\\\{\},fontsize=\small]
(\textcolor{blue}{:action} prepare_garage_car_exit
  \textcolor{gray}{; garage door is locked and closed,}
  \textcolor{gray}{;  and garage lights are off}
  \textcolor{blue}{:precondition} (\textbf{and} (garage_door_locked)
                     (\textbf{not} (garage_door_open))
                     (\textbf{not} (garage_lights_on)))
  \textcolor{blue}{:effect} (\textbf{and}
            \textcolor{gray}{; garage lights are turned on}
            (garage_lights_on)
            (\textbf{oneof}
              \textcolor{gray}{; a visual sensor in garage sets}
              \textcolor{gray}{;  off the alarm if car is gone}
              (garage_alarm_on)
              (\textbf{and}
                \textcolor{gray}{; the car is inside the garage}
                (\textbf{not} (garage_alarm_on))
                (have_fuel_level)))
            (\textbf{oneof}
              \textcolor{gray}{; garage door is malfunctioning}
              (garage_door_locked)
              (\textbf{and}
                \textcolor{gray}{; door unlocks successfully}
                (\textbf{not} (garage_door_locked))
                (\textbf{oneof}
                  \textcolor{gray}{; garage door is obstructed}
                  \textcolor{gray}{;  by some object}
                  (\textbf{not} (garage_door_open))
                  \textcolor{gray}{; garage door opens}
                  (garage_door_open))))))
\end{BVerbatim}
\caption{PDDL example for preparing to open a garage door, which demonstrates the various complexities of nested non-deterministic effects.}
\label{fig:pddl-example}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/effect_diagram_v2.pdf}
    \caption{Effect tree of the action in Figure \ref{fig:pddl-example}.}
    \label{fig:effect-example}
\end{figure}

As alluded to in the previous section, we can view the effect of an action as an \textit{and-or} tree (illustrated for our example in Figure \ref{fig:effect-example}). While this analogy is useful for some aspects, such as defining the realizations of an effect as $\realizations{}$, it is important to recognize the distinction from a Boolean formula represented as an \textit{and-or} tree: \textbf{the effect of an action is not a Boolean function to be evaluated}. The biggest ramification of this is that we evaluate the effect in a top-down manner (starting with the root) rather than bottom-up. We elaborate on this point further in Section \ref{ssec:complex_outcome_determination}. Also, note that unlike a common \textit{and-or} graph, we cannot simplify it by operations such as merging parent-child \textit{or-or} node relations or collapsing seemingly tautological subtrees (such as the bottom \textit{oneof} node in Figure \ref{fig:effect-example}), as each \textit{oneof} node has a unique determiner associated with it.


\subsection{State-Context Mapping}
\label{ssec:state-context-mapping}

\hide{          % ALL DONE %
\textbf{To discuss:}
\begin{itemize}
    \item Context is an assignment of values we maintain for execution, but the planner doesn't care about.
    \item State are the fluents that the planner knows and cares about.
    \item We find a reasonable abstraction so that the planner only needs to know the minimal amount of information to get by.
    \subitem * Based on the global example we can demonstrate it.
    \item The state and context should be aligned for all reachable states -- more on this when we talk about the role of determination.
    \item \textbf{(have-*)} fluents mapping to actual context variables. Only as an example (this paper doesn't need to go into the dialogue setting).
    \item \textbf{(maybe-have-*)} a controlled way of expressing uncertainties
\end{itemize}
}

Beyond the planner’s abstract view  of the world (the \textit{state}), a real-world system usually needs to retain contextual information needed for the practical execution of the plan. This brings the first key challenge that must be overcome: we need to track the correspondence between the state and the context. The execution state is a set of fluents that hold and are important for the planner to decide which actions can be executed. The context $C$ is an aligned assignment of values $C: \fluents \rightarrow Dom$, where $Dom$ is an arbitrary (and possibly open ended) domain.

The alignment can be illustrated with our running example: the state contains a fluent $\texttt{(have\_fuel\_level)} \in \fluents$ denoting the level of fuel in the car. From the planner's viewpoint, the only important result from preparing the car to exit the garage is whether the system knows the fuel level or not (regardless of its value). However, the fuel level itself may play a role in the execution and determination of other actions, so the context value associated with the fluent (e.g., $C(\texttt{(have\_fuel\_level)}) = 10L$) may become important. For example, there may be another action, \texttt{check\_fuel} that has a precondition \texttt{(have\_fuel\_level)} and non-deterministically results in either \texttt{(sufficient\_fuel)} or \texttt{(not (sufficient\_fuel))} (the former of which could act as a precondition for driving).

%
%Skipping for now, since our "have" example doesn't make sense with the "maybe" notion.
%
%When more fine-grained information about context values for planning is required, new fluents need to be added. E.g. if planner needs to select its actions based on confidence levels, ${maybe\_have\_location(src)}$ can be added and used for deciding whether the source location should be confirmed or not.

The advantage of splitting the execution information is twofold. 
First, it situates the planner at the right level of abstraction with the context maintained separately from the state.
Second, it allows an interconnection between the plan and complex objects (like a web call result, agent coordinates, etc.) which would be impractical to represent in the planning domain.
%
Maintaining the context alignment for all reachable states is one of the challenges in outcome determination, and is described further in Section~\ref{ssec:complex_outcome_determination}.



\subsection{Action Execution -vs- Determination}
\label{ssec:exec-vs-det}

\hide{          % ALL DONE %
\textbf{To discuss:}
\begin{itemize}
    \item General philosophy: split an action's execution into two phases; (1) is the execution of the action itself (system call, whatever), and (2) is the realization of the result.
    \item Phase (1) is the initiation of the action, and actually invokes whatever real-world process is happening.

    \item Both execution and determination can only view (TODO: updates should be also somewhat limited) the subset of the context / state that appears in the precondition: a guiding principle to avoid executor errors (model should reflect assumptions on execution / determination).
    \item TODO: I'm not sure whether context and state updates belong here or to the following subsection (assuming the later).
\end{itemize}
}

The aim of contingent plan execution is running action callbacks associated with each state to achieve a specified goal state.
However, in a non-deterministic world, an action can cause one of multiple effects in the state and context. 
%Therefore, an essential part of the plan execution is deciding which of the effects has happened, i.e. the outcome determination.
Moreover, in the real world, the effects may not be fully observable and may be too complex to be modeled perfectly.
Therefore, an essential part of the plan execution is deciding which of the effects best describes the real world change. This is the process of \emph{outcome determination}.

This leads us to a natural decomposition of action execution into two phases (steps 3 and 4 from Figure \ref{fig:architecture} respectively). First, running the function callback that implements the real process in the outside world (e.g. calling a web service), which gives the system a function call result (e.g., a response code with a payload of information from a web service).
Second, the outcome determination, which processes the function call result to update the execution state and context.
Note that the outcome determination is a complex multistep process described in detail in the following section.% Section~\ref{ssec:complex_outcome_determination}.
At a high level, the determination process involves running the appropriate callback functions in the appropriate order to establish what realization should be used to update the state of the world and the solution status.

The separation between action execution and outcome determination is not just conceptually attractive from the standpoint of clearly separating distinct functionality in the implementation; it also provides a natural means of encouraging better declarative models. With the evaluation of an effect focused on computing what has changed (as opposed to making additional changes to the real world), complex and error-prone action models are avoided in lieu of multiple actions, each with a clearly defined purpose. The core anti-pattern that is avoided is the strategy of embedding aspects of an agent policy directly within an action effect (e.g., if a determiner selects one branch, then further actuation occurs that influences the environment).

In theory, the callback function and outcome determiners could be given the entire state and context. 
However, such a practice would result in an error-prone and hard to debug system.
Therefore, \textit{only the context subset claimed in an action's precondition is accessible for the action execution}: $C_a = \{C(f) | f \in \pre a \}$. This drastically reduces the potential for model mismatch due to modeling errors between the planning view of state, and full view of context. Providing the full context and state would be akin to using global variables exclusively in software development -- a practice largely viewed to be error-prone and undesirable.


\subsection{Complex Outcome Determination}
\label{ssec:complex_outcome_determination}

\hide{          % ALL DONE %
\textbf{To discuss:}
\begin{itemize}
    \item Determination needs to find realization based on action effect specification (TODO reference to the PDDL example)
    \item Determination is a non-trivial task $\rightarrow$ decompose it to and-or graphs 
    \item Data revision (i.e. context updates) for the outcome determination
    \item Effective execution (parallelism) can be used thanks to the decomposed determination
    \item Outcome ranking as an approach to cope with Partial observability
    \subitem * Full action determinations can be driven by recursive rankings (with performance impact however) or with a limited look-ahead
    \subitem * "Outcome determination learning" can be defined with the rankings (TODO how deep want we go into it?)
    \item Visual example of the graph that mirrors a complex effect written in PDDL.
    \item Determination need not (and at times cannot) be done exhaustively -- instead you work top-down and determine only what needs to be.
    \item The state/context do not change until phase (2). This is why we need the assumption of non-overlapping or complex durative actions.
    \item Determination can be a long-running process in itself -- but the separation of execution (i.e., ``do something'') and realization (i.e., ``what's changed'') should be maintained. That is, in order to avoid escalating complexity of individual action specifications, and the potential for unforeseen side-effects, an action should correspond to at most one physical transition in the real-world setting.
\end{itemize}
}

The outcome determination is a fundamental part of action execution within a contingent plan. 
The role of determination is to decide which realization $r \in \realizations{a}$ of the action $a$ has occurred after the action callback $\exec{a}$.

The action realization $r$ is made up of $\add{r}$ and $\del{r}$ sets.
During the outcome determination, those sets are recursively calculated from the action effect tree, and use the $\determiner{}$ callbacks to compute these values for updating both the execution state and context.

\subsubsection{Recursive Effect Processing}
The effect tree consists of nodes with two kinds of operators.
First, the \textit{and} operator $\effand {\varphi}$ with sub-formulae ${\varphi_i}$ can be recursively calculated as:
\begin{gather*}
    \add{\effand {\varphi}}  = \bigcup_{\varphi_i} \add{\varphi_i}  \hspace{2em}
    \del{\effand {\varphi}}  = \bigcup_{\varphi_i} \del{\varphi_i}
\end{gather*}
Second, the \textit{or} operator $ \effoneof {\varphi} $ and its selected child $\varphi_j$   :
\begin{gather*}
    \add{\effoneof {\varphi} }  = \add{\varphi_j}
    \hspace{2em}
    \del{\effoneof {\varphi}}  = \del{\varphi_j}
\end{gather*} 
The effect tree leaves $\varphi_L$ directly define the $\add{\varphi_L}$ and $\del{\varphi_L}$ sets.
With this recursion defined, the action realization update sets are calculated as update sets for the effect's top-level root node.
%
The crucial part of outcome determination is the $ \effoneof {\varphi_j} $ selection. 
In practical systems, the selection can be a time consuming service call. 
For instance, the agent can use an outcome determiner that performs a remote service call to a deployed recognition model for detecting entities in a scene (e.g. one detecting whether there is an obstacle in the driveway or one detecting whether it is already dark outside to require headlights).
%The model recognizes intents and entities in user input (obtained during the previous action \textit{listen\_to\_command}) that the agent needs to decide how the state should be changed.
%
Such calls can take a long time to execute (due to network latency and complexity of the computation), and therefore exhaustive calculation over the whole tree (which can be full of such expensive calls) might not be suitable.

Thanks to the tree structure, effects can be processed top-down, evaluating only the nodes that can contribute to the realization. 
For example, each \textit{oneof} node needs only one sub-tree to be fully evaluated, and processing of that one sub-tree will only begin once the determiner for the \textit{oneof} node has identified that it is the right one to proceed with.
On the other hand, all of the sub-trees of an \textit{and} node must be evaluated, which can be done in parallel (recall that the resulting update sets are not contradicting by definition). This process can be captured by the following algorithm:

\makeatletter
\xpatchcmd{\algorithmic}{\itemsep\z@}{\itemsep=0.5ex plus2pt}{}{}
\makeatother

\begin{algorithm}
\caption{Parallel Nested Determination algorithm}\label{alg:parnes}
 \footnotesize
\begin{algorithmic}[1]
\Procedure{\textsc{ParallelNested}}{$node$}
\If{$node.type=leaf$}
    \State \textsc{ProcessLeaf}$(node)$
\ElsIf{$node.type=oneof$}
    \State $child = DET_{node}()$\Comment{Run determiner}
    \State \textsc{ParallelNested}$(child)$
\ElsIf{$node.type=and$}
    \State apply\_async(\textsc{ParallelNested}, node.children)
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

Note that on line 8, the children of an \textit{and} node are concurrently processed, while on lines 5-6, the determiner for a \textit{oneof} node is run until completion before recursing. Line 3 encapsulates the recursive $\add{}$ and $\del{}$ computation.


Retaining the full complexity of action effects thus gives us two key improvements in efficiency: (1) the ability to avoid evaluating sub-trees that correspond to outcomes a determiner deems did not occur; and (2) the ability to run determiners in parallel when they represent sibling sub-trees of an \textit{and} node in the effect graph.


\subsubsection{Dependencies Between Effects}
There is another consideration which makes our recursive tree structure necessary to leverage parallelism. Some of the determiners may be able to start evaluating only once some other determiners have finished executing. For instance, in our garage example, the status of the garage door being open or not is only relevant if the door is unlocked. In more extreme examples, a determiner may not be executable at all if its parent determiner did not resolve in a way that enables the child (i.e., having the right outcome selected). Such dependencies can prevent full parallel execution of all the determiners simultaneously in a flattened structure while our recursive tree structure does allow us to leverage at least partial parallelism in such cases.

\subsubsection{State and Context Updates}
With the realization update sets prepared, the new state after the action execution can be calculated as usual: $S_{i+1} = (S_i \setminus \del{r}) \cup \add{r}$.
%\begin{gather*}
%    S_{i+1} = (S_i \setminus \del{r}) \cup \add{r}
%\end{gather*} 

Context $C$ also has to be updated during the outcome determination. 
The new context values are produced by the determination process directly along the tree traversal described above (i.e., as part of the $\determiner{}$ callback functions), and can additionally make use of the $\exec{}$ action response.
%
Our running example demonstrates one possible update: the fuel level will be set during the determination process given the information computed by $\exec{\texttt{prepare\_garage\_car\_exit}}$.
%
%Various outcome determiners are expected to provide many types of context values. Example of an outcome determiner can be an entity extractor providing a specific entity type for the context and selecting $\varphi_i$ according to the entity presence in the function call result features $z$.
%
Formally, a realization $r \in \realizations{a}$ will have
%an associated set of
context updates $C_r$ defined as:
\begin{align*}
    \set{C(f) = val \st f \in \add{r}} \cup \set{C(f) = \bot \st f \in \del{r}}
\end{align*}

The assignment of $C(f) = val$ is defined by the determiner callback for the effect tree's leaf nodes, $\determiner{\varphi_f}$ (not all fluents have context necessary for execution, in which case we set $C(f) = \bot$). Notice that such updates force the precise alignment of context and state, which is necessary for the system to function properly during execution. 

%The fluents and context are updated solely from $\exec{}$ action response that can be understood as a measurement of real world objects.
%This way, we avoid complex (circular) dependencies between fluents and context values that can be hard to manage as shown in TODO.

Dependencies introduced by real world mechanics can cause difficulties for context value updates.
For instance, fluent \texttt{(have\_position)} and its context value $[x,y]$ may represent an agent position (and the validity of its reading).
Then, fluents like \texttt{(have\_x)} and \texttt{(have\_y)} and their context values $[x]$ and $[y]$ correspond to separate position sub-components.
An action changing a single sub-component for fluent \texttt{(have\_x)} must also update context value of \texttt{(have\_position)} which breaks action encapsulation and may lead to human errors during development.

Effective modeling of such real world dependencies is an interesting challenge that we keep for future work.


\subsubsection{Completing Determination}
Once we have completed the determination process for action $a$, we are left with a new state $s$, context $C$, and realization $r \in \realizations{a}$. Given the current node $n$ of the contingent plan, we compute the updated node as $n' = \edgemap{n}{r}$. The final step of the executor is to store all of the newly computed information ($s, C, n'$) in a centralized database (step 5 in Figure \ref{fig:architecture}). 



==> resources/plan4dial-paper-related.tex <==

\section{Related Work}
\label{sec:related}

%\ab{Partial draft copied and pasted from another draft. Needs work,
%  including more references and differences from our work.}
%   Previous work involving AI planning in
% dialogue systems includes mixed-initiative planning, with the
% capability of explaining the decisions of a planning system to the
% user
% ~\cite{DBLP:conf/sigdial/NothdurftBBBM15}.   %\citeauthor{cheong-et-al2014} ~\shortcite{cheong-et-al2014}
%focus on understanding a problem instance formulated in natural
%language. The problem is converted into a formal representation, which
%can be fed into a solver, such as CAD.

% Whole sentences can be generated word-by-word with AI planning
% techniques, as shown in work of~\intextcite{garoufi2010automated}.
% They were able to generate multiturn navigational commands followed by
% human users to reach a specified goal.

There are approaches to apply planning to interact with humans, e.g., using a pre-existing library of plans for dialogues \cite{Kuijpers1998}, 
facilitating mixed-initiative collaborative discourse \cite{Steedman07planningdialog},
modeling integrated behaviors \cite{AlbertLudwigs2008ACM},
and explaining decisions of the planner to the user \cite{DBLP:conf/sigdial/NothdurftBBBM15},
and assisting conversations \cite{DBLP:journals/aim/Ortiz18}. 
However, none of these approaches employ nondeterministic planning
to generate customized dialogue plans.

\hide{
\citeauthor{Kuijpers1998}~\shortcite{Kuijpers1998}
presented an approach where a pre-existing library of plans can be
used by an agent in a
dialogue. \citeauthor{Steedman07planningdialog}~\shortcite{Steedman07planningdialog}
advocated the use of planning to facilitate mixed-initiative
collaborative discourse.  In \cite{AlbertLudwigs2008ACM}, an algorithmic framework, namely, Continual
Collaborative Planning (CCP), is presented for modeling integrated behavior and which can naturally
blend physical and communicative actions. 
\citeauthor {Kominis2015}~\shortcite{Kominis2015} described methods developed for representing beliefs in single-agent planning to introduce a simple
formulation for handling beliefs in multi-agent settings. %\citeauthor{Petrick2013PlanningFS}~\shortcite{Petrick2013PlanningFS} describe an application of planning to task-based social interaction using a robot that must interact with multiple human agents. 
Epistemic planning can also be used for decision making in multi-agent situations with distributed knowledge and capabilities which can be based on Dynamic Epictemic Logic \cite{Bolander2017AGI}.
More recently,
\cite{DBLP:conf/sigdial/NothdurftBBBM15} described a system capable of
explaining the decisions of the planner to the
user. \intextcite{DBLP:journals/aim/Ortiz18} presented a holistic
approach to building conversational assistants which includes a
planning component to assist the interaction with human
users. However, none of these previous approaches employ planning
to generate customized dialog plans.
}

\citeauthor{garoufi2010automated}~\shortcite{garoufi2010automated}
employ deterministic planning for natural language sentence generation
about instructions to navigate to a location.
Their contexts are specific to navigation in
(simulated) physical environments. 
%and described an approach to generate multi-turn
%navigational commands to be followed by a human user in a
%conversational interface to achieve a specified goal.

\intextcite{black2014automated} represent persuasion dialogues as planning problems. 
While a planner can find optimal %persuasion
strategies, execution monitoring is simplified
due to the abstract nature of simulated dialogues.

Most of the work on dialogue planning is based on individual domains, including
conversation learners based on deep reinforcement learning \cite{Cuayahuitl16,SuGMRUVWY16a}.
Another example based on (deep) reinforcement learning is end-to-end dialogue
generation \cite{bhuwan2017,peng2018}. 

To the best of our knowledge,
%a few related art exists in the area of developing a composite task completion dialogue agent.
the work of \citeauthor{CTC2017}~\shortcite{CTC2017} is the first attempt to deal with composite tasks. 
Their approach combines deep reinforcement learning with hierarchical
task decomposition to train a dialogue manager. 
The dialogue manager consists of a top-level dialogue policy to select subtasks, a low-level dialogue policy to select primitive actions to complete a subtask,
and a global state tracker to ensure all
constraints across subtasks be satisfied. The approaches based on (deep) reinforcement learning
have an essential drawback of requiring a sufficient amount of training data. 
In practice, the amount of available data is typically too low to allow the training of good dialogue policies. 

\hide{
To the best of our knowledge, a few related art exists in the area of developing a composite task completion dialogue agent.
the first work in this area is presented in \intextcite{CTC2017}, which considers composite tasks as a set of subtasks that need to be fulfilled collectively.  The proposed method combines
deep reinforcement learning and hierarchical
task decomposition to train a composite task completion
dialogue agent. The dialogue manager consists of a top-level dialogue policy that selects subtasks, a low-level dialogue policy that selects primitive actions to complete a given subtask,
and a global state tracker that helps ensure all
cross-subtask constraints be satisfied. The main drawback of this work and all model based solutions for dialogue planning is that, they need sufficient amount of training data to train the dialogue policy.
However, the amount of available data is typically too low to allow the training of good dialogue policies. 
}

The approach of \citeauthor{petrick2013planning}~\shortcite{petrick2013planning}
monitors plan execution involving nondeterminism of dialogue systems. 
Their approach assumes deterministic behaviors of actions
and performs dynamic re-planning if inconsistencies between 
measurements and expected behaviors are observed (via various sensors). 
In contrast, our approach is more robust, since a plan it generates
accounts for nondeterminism explicitly and guarantees the existence of a path to a goal
from each state due to the use of FOND or MDP techniques.
In addition, our approach is easier for debugging the dialogue system, since it generates
a plan accounting for all possible outcomes before the plan is executed. 


\hide{
\intextcite{petrick2013planning} considered execution monitoring
issues that arise from nondeterminism of real-world dialogue systems.
Their proposed execution monitor expects deterministic behavior of
actions in the world and performs replanning if inconsistencies between
measurements and the expectations are observed (via various sensors). 
In contrast, our execution monitor accounts for nondeterminism
explicitly within the generated plan. Therefore, our plans can be
static and easier to debug.
}

\hide{
Examples of conversation learners include 
%Another direction of research is focused on using
(deep) reinforcement
learning
% based techniques 
for end-to-end dialogue
generation \cite{bhuwan2017,peng2018}. In contrast to our
%model-based
planning-based
approach, %training these data centric systems is costly and
%requires many interactions with human users.
their approach needs a large amount of training data obtained by many interactions with human users. 
}

Our work is conceptually close to (factored) POMDPs to manage spoken dialogue systems in various domains \cite{Williams2007,Thomson2007,bui2010}. 
However, their approaches are sensitive to the uncertainty inherent in
the spoken utterances and require considerable training to learn
good policies and thus drive the dialogue.
% in an effective manner.

%Other work exists on planning involving partial observability and nondeterminism, e.g., 
%\cite{Bolander2017AGI,Kominis2015}. 
%Embodying these approaches to fit well into our dialogue domain still remains open. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hide{

\jo{\textbf{Summary of articles 6 - 10} None of them is directly related to planning. I suggest we leave them all out of the related work except number 7 - \cite{DBLP:journals/aim/Ortiz18} which is already cited in the first paragraph of this article. \\

\begin{enumerate}
\item[6] Method for assigning a topic label to utterances in a chat log. Starts from noisy hand-crafted labeling and iteratively updates using reinforcement learning. They use rewards designed such that local topic continuity is enforced and global split into topics is such that utterances between topics are different. Meat is in sections 3.1 - 3.4. 

\item[7] From Christian: General argument for using all of the sub-modules possible in order to have an effective dialogue agent (including a need for a general planning component). Also points out that all of the sub-systems need to be designed with the holistic view in mind as it effects how they can inter-operate.

I would add that the author works in Nuance Communications and mentions a few practical examples. 

\item[8] Emphasizes the need for policy driven dialogues as opposed to end-to-end. It uses reinforcement learning for learning the policy which could be posed as an alternative/complementary approach to our work. Something like action preconditions must also be specified (execution mask in section II D). Based on state of the world (parsed entities ...) and the learned policy the algorithm selects next action and updates the policy according to the reward it receives (small negative for each step and big positive when user's goal is achieved). It employs a user simulator for training. 

\item[9] Historical overview of methods how to do conversational agents. Mostly concerned with end-to-end systems. 

\item[10] From Christian: Proposal for a user simulator. Also useful for the domain they have setup (movie booking with required / optional intents, etc). Code is available, so we could potentially use this as an example to model explicitly, or for automated model acquisition. 
\end{enumerate}

}

\subsection{Citations from Christian's Mendeley}

\cm{I haven't yet read through all of these, and there are some repeats from Adi's text, but so far these are the papers that I've identified that may be relevant. Most have links, but I have a PDF for all of them.}

\begin{enumerate}
  \item Srivastava, B. (2018). On Chatbots Exhibiting Goal-Directed Autonomy in Dynamic Environments, 588–590. Retrieved from http://arxiv.org/abs/1803.09789
  \item Feng, W., Zhuo, H. H., \& Kambhampati, S. (2018). Extracting Action Sequences from Texts Based on Deep Reinforcement Learning, 4064–4070. https://doi.org/arXiv:1803.02632v2
  \item Camilleri, G. (n.d.). Dialogue systems and planning, 1–8.
  \item Steedman, M., \& Petrick, R. (2007). Planning dialog actions. SIGdia 2007, (September), 265–272. Retrieved from http://homepages.inf.ed.ac.uk/steedman/papers/dialog/sigdial07.pdf
  \item Foster, M. E., \& Petrick, R. P. A. (2017). Separating representation, reasoning, and implementation for interaction management: Lessons from automated planning. Lecture Notes in Electrical Engineering, 999 LNEE, 93–107. https://doi.org/10.1007/978-981-10-2585-3$\_$7
  \item Takanobu, R., Huang, M., Zhao, Z., Li, F., Chen, H., Zhu, X., \& Nie, L. (2017). A Weakly Supervised Method for Topic Segmentation and Labeling in Goal-oriented Dialogues via Reinforcement Learning.
  \item Ortiz, C. L. (2018). Holistic Conversational Assistants, 88–90.
  \item Weisz, G., Budzianowski, P., Su, P.-H., \& Gašić, M. (2018). Sample Efficient Deep Reinforcement Learning for Dialogue Systems with Large Action Spaces, 1–14. Retrieved from http://arxiv.org/abs/1802.03753
  \item Mathur, V., \& Singh, A. (2018). The Rapidly Changing Landscape of Conversational Agents, 1–14. Retrieved from http://arxiv.org/abs/1803.08419
  \item Li, X., Lipton, Z. C., Dhingra, B., Li, L., Gao, J., \& Chen, Y.-N. (2016). A User Simulator for Task-Completion Dialogues. Retrieved from http://arxiv.org/abs/1612.05688
  \item Romero, O. J., Zhao, R., \& Cassell, J. (2017). Cognitive-inspired conversational-strategy Reasoner for socially-aware agents. IJCAI International Joint Conference on Artificial Intelligence, 3807–3813.
  \item Petrick, R. P. a, \& Foster, M. E. (2004). Planning for Social Interaction in a Robot Bartender Domain. Proceedings of the Twenty-Third International Conference on Automated Planning and Scheduling, 389–397. Retrieved from http://www.aaai.org/ocs/index.php/ICAPS/ICAPS13/paper/viewFile/6039/6208
  \item Casanueva, I., Budzianowski, P., Su, P.-H., Ultes, S., Rojas-Barahona, L., Tseng, B.-H., \& Gašić, M. (2018). Feudal Reinforcement Learning for Dialogue Management in Large Domains. Retrieved from http://arxiv.org/abs/1803.03232
  \item Black, E., Coles, A., \& Bernardini, S. (2014). Automated planning of simple persuasion dialogues. Lecture Notes in Computer Science (Including Subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics), 8624 LNAI, 87–104. https://doi.org/10.1007/978-3-319-09764-0$\_$6
  \item Garoufi, K., \& Koller, A. (2010). Automated planning for situated natural language generation. Acl, (July), 1573–1582.
  
  \ob{I've browsed through the following 6 papers. There's nothing that is really similar to what we do and nothing that uses automated planning in our sense. 
  
  Further notes under each paper, either very briefly from me, or from Christian.}
  \item Feng, W., Zhuo, H. H., \& Kambhampati, S. (2018). Extracting Action Sequences from Texts Based on Deep Reinforcement Learning. Retrieved from http://arxiv.org/abs/1803.02632
  \ob{
Feng et al (2018) extract sequences of actions from natural text (as in "The important thing to remember is not to heat up the rice, but keep it cold." -> keep(rice, cold)) using Reinforcement Learning. 

In our context, this could be useful for authoring an action-based dialogue system using natural language. }
  \item Raiman, J., \& Raiman, O. (2018). DeepType : Multilingual Entity Linking by Neural Type System Evolution.
  \ob{Integrates symbolic information (a type system) into NN reasoning. The system itself extracts the necessary structures. I'd say it's rather off-topic.}
  \item Ilievski, V., Musat, C., Hossmann, A., \& Baeriswyl, M. (2017). Goal-Oriented Chatbot Dialog Management Bootstrapping with Transfer Learning. Retrieved from https://arxiv.org/pdf/1802.00500.pdf
  \ob{An approach to help RL learning of dialogue policies by transfer learning from data rich domains.
  
 Christian's notes:
  
 General approach is to train a GO chatbot via RL, and then use the overlap with another domain to seed the learning for the new domain. They look at both the partial overlap setting, as well as domain extension (first domain is a subset of the next).

Section 4 seems to be the entire meat of the approach, and there isn't much. I guess it's something that need to be tried, but they don't do anything smart with the weights that carry over, do assume they already have the annotated overlap, don't operate on the NLU / NLG level (just the idealized semantic frame level), etc, etc.

The one thing that may be useful to take away from this paper are the domains that are used. Generally the accuracy is very poor, and a model-based approach should be able to accomplish far greater things.
}
  \item Azaria, A., Krishnamurthy, J., \& Mitchell, T. M. (2016). Instructable Intelligent Personal Agent. Proceedings of the 30th Conference on Artificial Intelligence (AAAI 2016), 2681–2689. Retrieved from http://ai2-website.s3.amazonaws.com/publications/LearnByInst.pdf
  
  \ob{Approach to learn new commands - a mapping NL sentence -> action sequence. No planning though.    
  
 Christian's notes:
  
Introduces a (traditional NLP) way of interacting with a domain-specific agent so that new commands can be learned. The scope is fairly narrow, but the general idea is a wonderful target -- interacting through natural language to teach an agent new skills.

The sentences are parsed using a specifically set up and learned grammar, and the key component is to identify the main entities so they can be lifted for generalization (e.g., other email targets).

A significant part of the work focuses on the user study, and all of the qualitative metrics that were lifted from the interaction.
  }
 
 \item Peng, B., Li, X., Gao, J., Liu, J., \& Wong, K.-F. (2018). Integrating planning for task-completion dialogue policy learning. Retrieved from http://arxiv.org/abs/1801.06176
    \ob{This certainly falls rather under RL than planning. What they call "planner" is a user-simulator that they use on some iterations instead of querying a real user to aid their RL and make it less expensive. No planning in our sense though.
    
    
    Further Christian's notes:
    
Their general approach is to do a bit of look-ahead during online conversations to improve the policy. The use of the word "planner" is extremely misleading here.

Essentially, their planner is a policy that is trained to mimic the end-users. This way, an on-the-fly simulation can be interleaved with the real dialogue, and mini segments of offline training can be done online.

Not quite sure what the model is that is being learned, but it appears as though the agent already has most of the components needed for model-based reasoning. The proposed approach also bootstraps with assumed offline generated training.

Another key point is that they do very little NL work (and provide little details as to how it's done). The NLU and NLG components are entirely missing, and the dialogue agent policy that is being built seems less than compelling -- major reason for this, is that (as far as I can tell), this problem would be trivial for a model-based planner to tackle. No need for RL, no need for deep nets. Etc.

Anyways, there's a good set of references, and simulation is criticized with valid references (which kind of contradicts what it is that they're doing).

  }
  \item Shah, P., Hakkani-Ur, D., Ur, G., \& Rastogi, A. (2017). Building a Conversational Agent Overnight with Dialogue Self-Play, (i). Retrieved from https://arxiv.org/pdf/1801.04871.pdf
    \ob{Christian's notes:
    
      This work is essentially dedicated to a new way for collecting
      data on annotated conversations. Instead of having humans
      converse with one another and then annotate with the slots and
      frames (or having others annotate), they flip this on its head
      and generate dialogue at the slot/frame level (using
      simulators), then have simple NLG create a crude approximation
      of a natural utterance, and /then/ have a turker paraphrase it
      (sanity checks done with crowdsourcing as well).

      It's basically a new way to do data collection, and seems to be
      smart about it. We could possibly use the domains in our own
      testing, but this falls under the camp of just simple dialogue
      generation end2end.  }
\end{enumerate}

} % end hide


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

==> resources/plan4dial-paper-reviews.tex <==

----------------------------

Paper ID: 5035

Title:    Generating Dialogue Agents via Automated Planning 
 


*** Metareview *** 

*** Review ***

•	Relevance: 5

•	Significance: 2

•	Originality: 3

•	Technical quality: 3

•	Clarity and quality of writing: 5

•	Scholarship: 6

•	Overall score: 3

•	Confidence: 6

- Comments to Authors :

This paper discusses the use of automated planning to generate dialogue agents. The authors discuss their experiences in using existing planning techniques to generate dialogue plans. These dialogue plans can contain dialogue actions (that send a message to a user) and service actions (that include things like system checks and calls to external services).

I’m confused about what the contribution here is meant to be. There is some discussion around how a dialogue plan is run and monitored, but this seems to be implementation level considerations and it’s not clear to me that this represents a research contribution. There is also some discussion about how a specific domain has been modelled as a planning problem, but I don’t see how someone from the community might use this since (1) the lack of formal detail means the approach is not reproducible and (2) the authors provide some specific examples relevant to their domain, rather than specifying a general approach that one could apply to a range of problem domains. In summary, I don’t believe this paper is appropriate for an ijcai audience, since it doesn’t provide a significant contribution for the AI community. It may be more appropriate to consider a venue that focusses on the applications of AI. Some more comments follow.

The authors talk about FOND planning, MDPs and PDDL, but it’s not clear how these relate to, or are used by, the approach. Is the problem modelled as a FOND planning problem or as an MDP? Section 6 focusses on PDDL, but in Section 7, it appears that the authors also formulate their problem as an MDP (presumably not in PDDL?).

Standard PDDL does not directly model non-deterministic actions; it’s not clear how this is dealt with here. Is a variant of PDDL being used? If so which one?

We aren’t told which off the shelf domain-independent planner is being used.

A reference for PDDL should be given.

The reference [Black et al., 2014] is superseded by: Elizabeth Black, Amanda J. Coles & Christopher Hampson. Planning for persuasion. 16th International Conference on Autonomous Agents and Multiagent Systems (AAMAS). 2017.



 

*** Review ***

•	Relevance: 8

•	Significance: 3

•	Originality: 5

•	Technical quality: 3

•	Clarity and quality of writing: 8

•	Scholarship: 7

•	Overall score: 4

•	Confidence: 6 

- Comments to Authors :

The paper presents an automatic approach to generate high-level plans for orchestrating operations of a dialogue system. This is done using an off-the-shelf MDP planner, in which operators are defined as an abstraction of operations that a full conversational dialogue system would need to perform to accomplish a dialogue goal. I believe the topic fits well within the scope of the conference. 

 

The paper is well written as a whole, the applications are interesting and the motivation of the paper is sound. The work seems to be well situated in the literature, although a clearer comparison with what other dialogue systems use for  task manager methods should be emphasised. I have however some concerns with the significance and technical quality of this paper.  

 

The focus of the work appears to be a knowledge engineering approach for a plan domain. A set of types of actions orchestrating a dialogue system are encoded into an existing MDP planning system. Although this is a useful and interesting application of automated planning, I found the significance of the contribution somewhat limited to an application of existing work, in a novel area. The planning approach to orchestrate a dialogue may indeed bring some advantages over more static structures but it is not entirely clear whether there are any advantages from a system perspective. These advantages are indeed useful for the designer, as shown by the larger amount of possibilities generated in the results. However, the results are somewhat limited to indicating that with a well constructed planning domain, we are able to obtain many potential plans, in different domains but not necessarily what this means comparing to other systems. The paper does a good comparison with other systems presenting some good pointers at the end of the paper  such as termination verification, but there is no theoretical or empirical evaluation of this approach.  

 

Some additional considerations could also be made on whether there is a need to construct a plan; assuming that the domain is well defined, we could for example have just a simple decision at each step. Perhaps some further discussion of the advantages of the approach should be proposed. Certainly, constructing plans allows for a choice of an optimal plan, which might help leading the conversation, but it is unclear what it is intended for an optimal plan in this work. In other words, the heuristic used is based on equal probabilities among all actions which seems to lead to very few advantages. Defining an optimal policy for a plan involving user responses may be complex but attempting a few would be useful. For example, a plan that finishes with the user interrupting will have the same priority as a plan that finishes with reaching a goal in the example (assuming no cycles). Perhaps the system should try to achieve the latter first. 

 

Another area of concern is the typology of actions proposed in the definition of plans. Such typology is intended to be at a ‘high/abstract-level’ and claimed to be general, however although it removes some context dependencies related to the dialogue itself, the system operations must be contextualised.  This procedure of abstraction however does not seem to be rigorously defined, which leaves doubts on what is required to be encoded and what is not required.   In fact it seems an ad-hoc approach as deciding when an action can be performed may be conditional to the outcomes of a previous action and of the available actions/services in the system and so it seems hard to create a general model prescribing the level of details required. For example, would a simple planning domain with very abstract actions be accepted in the current approach? e.g. receive user response, interpret response, send response to user.  It seems to me that this “knowledge-engineering” approach to defining plan domains for dialogue requires a set of clear guidelines or an ontological/hierarchical representation of the tasks that clearly specifies when we have enough details and a sufficient level of abstraction. Also there are clearly trade-offs on the abstraction of these actions and the complexity of the transformers that should be evaluated. 

 

Another area of concern within this paper is the technical quality of the approach introduced. The paper starts well describing the approach at a high level. However, the technical sections seem to be a mix of formal and informal features, some of those also “auxiliary” parts of the system that perhaps are not required to be discussed in detail, in favour of more details of the planning domains.

 

The core part of the paper, the formulation of planning domains, would benefit from much more formal technical details. Planning graphs are defined twice in section 2 and 3 with different notation. After there is no reference to the technical definitions, which instead would be useful to clarify the approach used for engineering these planning domains. Examples of resulting action definitions, and/or alternative plans would be useful. In particular highlighting whether there are characteristics of the dialogue vs service actions that are apparent in their operator structure. As per the point above, a more structured or guided definition of abstraction should be given for these actions. 

 

Section 5 is quite hard to interpret and it would be important to give precise definitions or just to remove them. Some examples include “context”: what are variables W? what is their domain or scope? How do they get updated? Do they have a value associated?  Which of those variables are used in the planning domain, and how is it decided? “NLU”: what is the relationship between intent and entities? Are values used in any way in the plans? 

The transformers are an interesting component, and it would appear that they require some complex mapping to transform a simple statement such as update user profile to an actionable task, it would also be good to discuss what are the drawbacks of this approach.   

 

While I find the application of a non-deterministic planning domain interesting and clearly providing promising results, I think more focus of the contribution and advantages of the approach and clarity in its technical presentation would be useful to improve the paper. 



 


 

*** Review ***

•	Relevance: 8

•	Significance: 4

•	Originality: 6

•	Technical quality: 5

•	Clarity and quality of writing: 8

•	Scholarship: 8

•	Overall score: 4

•	Confidence: 9 

- Comments to Authors :

The authors propose in this paper an application of automated planning for dialogue generation. This is done by encoding the dialogue planning problem as a FOND. This application of planning has been explored in the past, but offers interesting challenges in the planning problems generation, and in interfacing different technologies together (speech recognition, planning, ...).

The paper is well written, but there are certain aspects of the paper that are not clearly described, and can confuse the reader. This includes the motivation for using an independent planner, but also the modelling of the problems.

The motivations include "calls to external services" and "handling contingencies". This rises the question if the time constraints are taken into account and how; while the second point seems to go in the direction of contingent Planning, rather than FOND. About the latter, embedding observations (that can be included in the form of speech acts) can greatly simplify the task of the planner, reducing the belief state, and reaching the goal quicker. In fact, the "full observability" assumption that lies behind FOND planning is rather strong in such domains. The user's intentions are not always clear, and the planning problem can includes contingencies by itself. This need is reflected in the example of sec. 6, where a train has to be recommended to the user. Having the possibility to indicate preferences about the travel (e.g. "Do you prefer travelling before of after 1pm?"; "Do you want to arrive at 4pm?"") can shorten the plan length, and allow the planner to restrict the timetable goals, while having an knowledge representation of the user.

Here the non-deterministic actions are considered "useful to respond in different ways in a given state", but they are not considered as part of the reasoning process itself. It is indeed possible to include them in the domain description, in order to reason about the non-determinism of the problem, at a cost of changing the planning paradigm. In the example PDDL files, it is confirmed that some fluents are mutually exclusive, so reasoning in terms of "oneof" clauses could be helpful in those cases (unless full observability is assumed, as said, but this is a very strong assumption for such problems where even the user's intentions aren't determined).

The planning model is never explicated. A reader in the automated planning community would expect to read a formal description in terms of:

F, a set of fluents
A, a set of actions
I, the initial state(s)
G, the goal state(s)
c(A), action costs
The PDDL sources help greatly in that: I highly appreciated their availability because they helps to understand the approach better and the community to test the benchmarks. However, it is a formal definition that is needed, otherwise it's not clear how the planning problems are described, and if it is done in an automated way. Moreover, in sec. 4,5,6 the relevance of the fluents to the goal is obscure, in particular because it is written that the PDDL model only describes an abstraction of the problem.

From the examples shown (both PDDL and in the paper), the domains seem quite simple, with a solution plan made by 2 or 3 actions in sequence (this is somewhat contradicted in sec. 7, when it is written that plans have an average length of 30 actions possibly). Is there really the need of an general purpose planner for that, or even of using automated planning at all? I understand that dialogue planning problems can vary depending of the user case, which justifies the usage of an independent planner. However, such planning problems seem to have a commons structure that might be hardcoded (or fed to a domain specific planner) for sake of effectiveness.

The generation of the planning problems should deserve a larger place. In fact, the planning process is quite trivial, while the interest of the application resides in the connection of different technologies. A dialogue planning problem is expected to be generated on-the-fly, based on the user's requests.

In trip planning, it would be better to specify if a replanning episode is triggered by the user's choice. If a replan is triggered, then what are the new goals and initial states should be indicated.



== Minor stuff ==

- The figure 1 is too small: unreadable if printed

- Sec. 7 Plans are generally described in terms of "actions", not "states"

 


 

*** Review ***

•	Relevance: 9

•	Significance: 4

•	Originality: 7

•	Technical quality: 3

•	Clarity and quality of writing: 3

•	Scholarship: 7

•	Overall score: 4

•	Confidence: 8 

- Comments to Authors :

This article presents an architecture in which AI planning is used to plan the dialogue between the system and its users. The authors present the different modules in the architecture and focus on how planning is used within it.

The paper is well written and easy to follow. The content is interesting, and I agree with the authors that planning could be critical in making a dialogue system more effective and attuned to the users’ need. Surprisingly, there is not much research on this topic and this paper positions itself well in trying to fill this gap. 

Having said that, this paper gives only a high-level view of the system. It is impossible to understand the details by reading it, which makes it difficult to assess it. The paper is probably more suitable for a journal venue where all the modules can be described in depth as well as their interconnection and the different applications. Alternatively, the authors should focus on planning, leaving out the rest of the modules. PDDL models need to be included in the text as well as details of the planning mechanism. I don’t find the evaluation particularly compelling. User studies need to be used to assess the effectiveness of the system as it is not enough to show the architecture is capable of generating dialogue.

Other minor points are:

- It seems that the system requires anticipating the users’ moves. Is this realistic? How do the authors gather possible users’ speech acts? 

- The rationale behind how to choose a career for a given user is not provided.


==> sections/inspection-model.tex <==

\newpage
\appendix
\section{PDDL Model for Car Inspection Domain}
\label{appendix:example}

Here we provide the full PDDL abstraction generated for the Car Inspection domain presented in the paper (cf. Figure \ref{fig:car-inspection-log}). Recall that this domain and problem is synthesized automatically from the specification in the Model Acquisition Interface. As such, it is common to see repeated structure throughout the action schema.

\subsection{Domain File}
\begin{Verbatim}[framesep=5mm,commandchars=\\\{\}]
(define
    (domain Car-Inspection)
    (:requirements :strips :typing)
    (:types )
    (:constants
      
    )

    (:predicates 
        (have_spark_plug_status)
        (maybe-have_spark_plug_status)
        (have_break_pad_status)
        (maybe-have_break_pad_status)
        (have_user_initiative_message)
        (maybe-have_user_initiative_message)
        (have_clutch_seal_tightness_status)
        (maybe-have_clutch_seal_tightness_status)
        (have_pass_status_options)
        (maybe-have_pass_status_options)
        (have_oil_status)
        (maybe-have_oil_status)
        (user_initiative)
        (have_message)
        (maybe-have_message)
        (GOAL)
        (STARTED)
        (can-do_dialogue-disambiguation-state-message)
        (can-do_dialogue-disambiguation-end_conversation)
        (can-do_dialogue-disambiguation-ask-for_spark-plug)
        (can-do_dialogue-disambiguation-ask-for_break-pad)
        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
        (can-do_dialogue-disambiguation-ask-for_oil-level)
        (can-do_dialogue-disambiguation-start_conversation)
    )
    (:action dialogue-disambiguation-state-message
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-state-message)
                (have_message)
                (not
                    (maybe-have_message)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-state-message
                (outcome state-message-outcome-fallback__
                    (and
                        (not
                            (have_message)
                        )
                        (not
                            (maybe-have_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
            )
    )
    (:action dialogue-disambiguation-end_conversation
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-end_conversation)
                (have_oil_status)
                (not
                    (maybe-have_oil_status)
                )
                (have_clutch_seal_tightness_status)
                (not
                    (maybe-have_clutch_seal_tightness_status)
                )
                (have_break_pad_status)
                (not
                    (maybe-have_break_pad_status)
                )
                (have_spark_plug_status)
                (not
                    (maybe-have_spark_plug_status)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-end_conversation
                (outcome end_conversation-outcome-fallback__
                    (and
                        (GOAL)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
            )
    )
    (:action dialogue-disambiguation-ask-for_spark-plug
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-ask-for_spark-plug)
                (not
                    (user_initiative)
                )
                (not
                    (have_spark_plug_status)
                )
                (not
                    (maybe-have_spark_plug_status)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-ask-for_spark-plug
                (outcome ask-for_spark-plug_initiative-switch__
                    (and
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (user_initiative)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome ask-for_spark-plug_detected__check-pass_status_options-eq-found
                    (and
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (have_spark_plug_status)
                        (not
                            (maybe-have_spark_plug_status)
                        )
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
                (outcome ask-for_spark-plug_help-local-options__
                    (and
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
            )
    )
    (:action dialogue-disambiguation-ask-for_break-pad
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-ask-for_break-pad)
                (not
                    (user_initiative)
                )
                (not
                    (have_break_pad_status)
                )
                (not
                    (maybe-have_break_pad_status)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-ask-for_break-pad
                (outcome ask-for_break-pad_initiative-switch__
                    (and
                        (user_initiative)
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome ask-for_break-pad_detected__check-pass_status_options-eq-found
                    (and
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (have_break_pad_status)
                        (not
                            (maybe-have_break_pad_status)
                        )
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
                (outcome ask-for_break-pad_help-local-options__
                    (and
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
            )
    )
    (:action dialogue-disambiguation-ask-for_clutch-seal-tightness
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                (not
                    (user_initiative)
                )
                (not
                    (have_clutch_seal_tightness_status)
                )
                (not
                    (maybe-have_clutch_seal_tightness_status)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-ask-for_clutch-seal-tightness
                (outcome ask-for_clutch-seal-tightness_initiative-switch__
                    (and
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (user_initiative)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome ask-for_clutch-seal-tightness_detected__check-clutch_seal_tightness_status-eq-found
                    (and
                        (have_clutch_seal_tightness_status)
                        (not
                            (maybe-have_clutch_seal_tightness_status)
                        )
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (have_clutch_seal_tightness_status)
                        (not
                            (maybe-have_clutch_seal_tightness_status)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
                (outcome ask-for_clutch-seal-tightness_help-local-options__
                    (and
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
            )
    )
    (:action dialogue-disambiguation-ask-for_oil-level
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-ask-for_oil-level)
                (not
                    (user_initiative)
                )
                (not
                    (have_oil_status)
                )
                (not
                    (maybe-have_oil_status)
                )
                (STARTED)
            )
        :effect
            (labeled-oneof resolve-ask-for_oil-level
                (outcome ask-for_oil-level_initiative-switch__
                    (and
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (user_initiative)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome ask-for_oil-level_detected__check-oil_status-eq-found
                    (and
                        (have_oil_status)
                        (not
                            (maybe-have_oil_status)
                        )
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (have_oil_status)
                        (not
                            (maybe-have_oil_status)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
                (outcome ask-for_oil-level_help-local-options__
                    (and
                        (have_message)
                        (not
                            (maybe-have_message)
                        )
                        (can-do_dialogue-disambiguation-state-message)
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (not
                            (can-do_dialogue-disambiguation-start_conversation)
                        )
                    )
                )
            )
    )
    (:action dialogue-disambiguation-start_conversation
        :parameters ()
        :precondition
            (and
                (can-do_dialogue-disambiguation-start_conversation)
                (have_user_initiative_message)
                (not
                    (maybe-have_user_initiative_message)
                )
                (user_initiative)
            )
        :effect
            (labeled-oneof resolve-start_conversation
                (outcome start_conversation_what__
                    (and
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_initiative-switch__
                    (and
                        (not
                            (user_initiative)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_break-pad__check-pass_status_options-eq-found
                    (and
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (have_break_pad_status)
                        (not
                            (maybe-have_break_pad_status)
                        )
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_spark-plug__check-pass_status_options-eq-found
                    (and
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (have_spark_plug_status)
                        (not
                            (maybe-have_spark_plug_status)
                        )
                        (have_pass_status_options)
                        (not
                            (maybe-have_pass_status_options)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_clutch-seal-tightness__check-clutch_seal_tightness_status-eq-found
                    (and
                        (have_clutch_seal_tightness_status)
                        (not
                            (maybe-have_clutch_seal_tightness_status)
                        )
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (have_clutch_seal_tightness_status)
                        (not
                            (maybe-have_clutch_seal_tightness_status)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_oil__check-oil_status-eq-found
                    (and
                        (have_oil_status)
                        (not
                            (maybe-have_oil_status)
                        )
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (have_oil_status)
                        (not
                            (maybe-have_oil_status)
                        )
                        (STARTED)
                        (can-do_dialogue-disambiguation-state-message)
                        (can-do_dialogue-disambiguation-end_conversation)
                        (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        (can-do_dialogue-disambiguation-ask-for_break-pad)
                        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        (can-do_dialogue-disambiguation-ask-for_oil-level)
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
                (outcome start_conversation_fallback__
                    (and
                        (have_user_initiative_message)
                        (not
                            (maybe-have_user_initiative_message)
                        )
                        (STARTED)
                        (not
                            (can-do_dialogue-disambiguation-state-message)
                        )
                        (not
                            (can-do_dialogue-disambiguation-end_conversation)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_spark-plug)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_break-pad)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
                        )
                        (not
                            (can-do_dialogue-disambiguation-ask-for_oil-level)
                        )
                        (can-do_dialogue-disambiguation-start_conversation)
                    )
                )
            )
    )
)
\end{Verbatim}

\subsection{Problem File}
\begin{Verbatim}[framesep=5mm,commandchars=\\\{\}]
(define
    (problem Car-Inspection_problem)
    (:domain Car-Inspection)
    (:objects
    )
    (:init
        (have_user_initiative_message)
        (user_initiative)
        (can-do_dialogue-disambiguation-state-message)
        (can-do_dialogue-disambiguation-end_conversation)
        (can-do_dialogue-disambiguation-ask-for_spark-plug)
        (can-do_dialogue-disambiguation-ask-for_break-pad)
        (can-do_dialogue-disambiguation-ask-for_clutch-seal-tightness)
        (can-do_dialogue-disambiguation-ask-for_oil-level)
        (can-do_dialogue-disambiguation-start_conversation)
    )
    (:goal
        (and
            (GOAL)
        )
    )
)
\end{Verbatim}

